LION: Lidar-Inertial Observability-Aware Navigator for Vision-Denied Environments

State estimation for robots navigating in GPS-denied and perceptually-degraded environments, such as underground tunnels, mines and planetary subsurface voids, remains challenging in robotics. Towards this goal, we present LION (Lidar-Inertial Observability-Aware Navigator), which is part of the state estimation framework developed by the team CoSTAR for the DARPA Subterranean Challenge, where the team achieved second and first places in the Tunnel and Urban circuits in August 2019 and February 2020, respectively. LION provides high-rate odometry estimates by fusing high-frequency inertial data from an IMU and low-rate relative pose estimates from a lidar via a fixed-lag sliding window smoother. LION does not require knowledge of relative positioning between lidar and IMU, as the extrinsic calibration is estimated online. In addition, LION is able to self-assess its performance using an observability metric that evaluates whether the pose estimate is geometrically ill-constrained. Odometry and confidence estimates are used by HeRO, a supervisory algorithm that provides robust estimates by switching between different odometry sources. In this paper we benchmark the performance of LION in perceptually-degraded subterranean environments, demonstrating its high technology readiness level for deployment in the field.

==> sections/architecture.tex <==
In this section we briefly present the localization architecture in which LION is used. 
LION is one of the odometry methods used by HERO \cite{santamaria2019towards} (Heterogeneous Redundant Odometry), a switching logic used to multiplex different odometry sources (for example  \ac{WO}, \ac{VIO}, \ac{TIO}), and selected one of them according to the reliability of their output as state estimate for the cascaded planner/controllers. The reliability of each odometry source is evaluated via a confidence score (e.g. covariance of the estimate, output rate of the method...) which informs the switching logic (also called \textit{resiliency} logic) on which method to use. One of the confidence metrics used to evaluate the reliability of LION is based on multiple elements, which include its output rate, the detection of the potential failures in its inputs (Lidar and IMU), and the geometric observability score detailed in Section \ref{sec:observability}.  
LION has been designed to be a state estimation method, whose main goal is to provide an high-rate output to the downstream algorithms. As such, it does not build any map and does not perform any loop closures, and thus its inertial reference frame will slowly drift over time. The slow drifts in the output of LION are compensated by mapping strategy \cite{Ebadi20lamp} running within the localization framework.
